Classification of Natural Language Processing Techniques for Requirements Engineering

Research in applying natural language processing (NLP) techniques to requirements engineering (RE) tasks spans more than 40 years, from initial efforts carried out in the 1980s to more recent attempts with machine learning (ML) and deep learning (DL) techniques. However, in spite of the progress, our recent survey shows that there is still a lack of systematic understanding and organization of commonly used NLP techniques in RE. We believe one hurdle facing the industry is lack of shared knowledge of NLP techniques and their usage in RE tasks. In this paper, we present our effort to synthesize and organize 57 most frequently used NLP techniques in RE. We classify these NLP techniques in two ways: first, by their NLP tasks in typical pipelines and second, by their linguist analysis levels. We believe these two ways of classification are complementary, contributing to a better understanding of the NLP techniques in RE and such understanding is crucial to the development of better NLP tools for RE.

==> Tables/Unused/tab-high-level-nlp.tex <==
\begin{table*}[ht!]

\caption{Classifying NLP Techniques by Level of Analysis (Higher Levels).}
\label{tab:highlevel}

\footnotesize
\resizebox{\textwidth}{!}{% use resizebox with textwidth

\begin{tabular}{|l|l|l|}
\hline
\textbf{Analysis Level} &
  \textbf{NLP Techniques} &
  \textbf{Meaning} \\ \hline
\multirow %{6}{*}
{\begin{tabular}[c]{@{}l@{}}\textbf{Word-Level} \\ \textbf{Semantic}\end{tabular}} &
  Similarity Analysis &
  \begin{tabular}[c]{@{}l@{}}Measures the similarity between two or more chunks of text based \\ on their syntactic structure or semantic content.\end{tabular} \\ 
 \cline{2-3} 
 &
  Named Entity Recognition (NER) &
  \begin{tabular}[c]{@{}l@{}}Classifying named entities from text into pre-defined categories or \\ classes such as the names of persons, organizations, locations, etc.\end{tabular} \\ 
  \cline{2-3} 
  &
  Semantic Role Labelling (SRL) &
  \begin{tabular}[c]{@{}l@{}}Identifying semantic roles in a sentence.\end{tabular} \\ 
  \cline{2-3} 
 &
  Latent Semantic Analysis &
  \begin{tabular}[c]{@{}l@{}}Analysing relationships between a set of documents and the terms \\ they contain by producing a set of concepts related to the documents \\ and terms.\end{tabular} \\ \cline{2-3} 
 &
  Topic Modelling &
  \begin{tabular}[c]{@{}l@{}}Recognizing the words from the topics present in the document or \\ collection of documents.\end{tabular} \\ \cline{2-3} 
 &
  Word Sense Disambiguation &
  Identifying which sense (meaning) of a word is used in a sentence. \\ \cline{2-3} 
 &
  Word Embedding &
  \begin{tabular}[c]{@{}l@{}}Word representation that allows words with similar meaning to have \\ a similar representation.\end{tabular} \\ \hline
  
\multirow%{4}{*}
{\begin{tabular}[c]{@{}l@{}}\textbf{Sentence-Level} \\ \textbf{Semantic} \end{tabular}} &
  Semantic Patterns &
  \begin{tabular}[c]{@{}l@{}}Semantic structures for identifying the relationships between sentence \\ components.\end{tabular} \\ \cline{2-3} 
 &
  Semantic Rules &
  \begin{tabular}[c]{@{}l@{}}Set of rules for semantically analysing the relations between sentence \\ components.\end{tabular} \\ \cline{2-3} 
 &
  Case Grammar &
  \begin{tabular}[c]{@{}l@{}}Linguistic analysis of functional relationships between noun phrases \\ and verbs.\end{tabular} \\ \cline{2-3} 
  &
  Semantic Frames &
  \begin{tabular}[c]{@{}l@{}}Description of a set of semantic roles (e.g., agent, place, time, duration) \\ and their interactions.\end{tabular} \\ \cline{2-3} 
 &
  Knowledge Graph &
  \begin{tabular}[c]{@{}l@{}}Stores inter-linked descriptions of entities – objects, events, situations \\ or abstract concepts.\end{tabular} \\ \hline
\multirow%{2}{*}
{\textbf{Discourse}} &
  Anaphora Resolution &
  Resolving what a pronoun, or a noun phrase refers to. \\ \cline{2-3} 
 &
  Coreference Resolution &
  Finding all expressions that refer to the same entity in a text. \\ \hline
\end{tabular}

}
\end{table*}


==> Tables/Unused/tab-low-level-nlp.tex <==
\begin{table*}[ht!]

\caption{Classifying NLP Techniques by Level of Analysis (Lower Levels).}
\label{tab:lowerlevel}

\footnotesize

\resizebox{\textwidth}{!}{% use resizebox with textwidth
\begin{tabular}{|l|l|l|}
\hline
\textbf{Analysis Level} &
  \textbf{NLP Techniques} &
  \textbf{Meaning} \\ \hline
\multirow%{2}{*}
{\textbf{Morphology}} &
  Stemming &
  Reducing inflected words to their word stem, base or root form. \\ \cline{2-3} 
 &
  \begin{tabular}[c]{@{}l@{}}Stop-Word Removal\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Removing commonly used words before or after processing of \\ NL data (text).\end{tabular} \\ \hline
\multirow%{12}{*}
{\textbf{Lexical}} &
  \begin{tabular}[c]{@{}l@{}}N-gram \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Predicating probabilistic language model for the next item in a \\ text sequence.\end{tabular} \\ \cline{2-3} 
 &
  Lemmatization &
  \begin{tabular}[c]{@{}l@{}}Removing inflectional endings of words to return the base or \\ dictionary form of a word.\end{tabular} \\ \cline{2-3} 
 &
  Text Segmentation &
  \begin{tabular}[c]{@{}l@{}}Dividing a string of written language into its component \\ sentences based on lexical or syntactic features.\end{tabular} \\ \cline{2-3} 
 &
  Frequency Analysis &
  \begin{tabular}[c]{@{}l@{}}Analysing the frequencies of words or terms in a certain context \\ and producing probabilistic data.\end{tabular} \\ \cline{2-3} 
 &
  Tokenization &
  \begin{tabular}[c]{@{}l@{}}Breaking a stream of text into words, phrases, symbols, or other \\ meaningful tokens.\end{tabular} \\ \cline{2-3} 
 &
  TF-IDF &
  \begin{tabular}[c]{@{}l@{}}Reflects how important a word is to a document in a collection \\ or corpus.\end{tabular} \\ \cline{2-3} 
 &
  Bag-of-Words (BOW) &
  \begin{tabular}[c]{@{}l@{}}Extracts features from text documents as  a sparse vector of \\ occurrence counts of word.\end{tabular} \\ \cline{2-3} 
 &
  Frequency Profiling &
  \begin{tabular}[c]{@{}l@{}}Provides a quantifiable characterization and classification of \\ lexical material in terms of corpus-based frequency measures.\end{tabular} \\ \cline{2-3} 
 &
  Occurrences Analysis &
  \begin{tabular}[c]{@{}l@{}}Clustering the words without breaking the links with semantic \\ analysis. It deals with the concordances between words and \\ not only with their number of occurrences.\end{tabular} \\ \cline{2-3} 
 &
  Co-location Analysis &
  \begin{tabular}[c]{@{}l@{}}Analysing a sequence of lexical terms that co-occur more often \\ together and established through repeated context-dependent use.\end{tabular} \\ \cline{2-3} 
 &
  \begin{tabular}[c]{@{}l@{}}Concordances \\ Analysis\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Calculating the occurrences of a word, together with some \\ context.\end{tabular} \\ \cline{2-3} 
 &
  Lexical Affinity &
  \begin{tabular}[c]{@{}l@{}}Measuring the distance between words (as concepts) based on \\ lexicalized resources e.g. WordNet\end{tabular} \\ \hline
\multirow%{6}{*}
{\textbf{Syntactic}} &
  POS Tagging &
  \begin{tabular}[c]{@{}l@{}}Processing a sequence of words to identify its word classes or \\ lexical categories.\end{tabular} \\ \cline{2-3} 
 &
  Dependency Parsing &
  \begin{tabular}[c]{@{}l@{}}Analysing the grammatical structure of a sentence based on the \\ dependencies between the words in a sentence.\end{tabular} \\ \cline{2-3} 
 &
  Chunking &
  \begin{tabular}[c]{@{}l@{}}Analysing a sentence by first identifying its constituent parts \\ then linking them to higher order units that have discrete \\ grammatical meanings.\end{tabular} \\ \cline{2-3} 
 &
  Regular Expression &
  \begin{tabular}[c]{@{}l@{}}Using a search pattern to match one or more characters within \\ a string.\end{tabular} %\\ \cline{2-3} &
  %Link Grammar &
  %\begin{tabular}[c]{@{}l@{}}Constructing relations between pairs of words.
 %\end{tabular} 
 \\ \cline{2-3} 
 &
  Constituency Parsing &
  \begin{tabular}[c]{@{}l@{}}Analyzing sentences by breaking down them into sub-phrases \\ or constituents.\end{tabular} \\ \hline
\end{tabular}
}
\end{table*}

